Dumb RIS-Assisted Random Beamforming for Energy Efficiency Enhancement of Wireless Communications

Energy efficiency (EE) is one of the most important metrics for the beyond fifth generation (B5G) and the future sixth generation (6G) wireless networks. Reconfigurable intelligent surface (RIS) has been widely focused on EE enhancement for wireless networks because it is power-saving, programmable, and easy to be deployed. However, RIS is generally passive and thus difficult to obtain corresponding full channel state information (CSI), which severely impacts the EE enhancement of RIS-assisted wireless communications. To solve this problem, in this paper we propose the new single-active-antenna combined RIS transmitter structure, which can replace traditional multiple antennas to reduce hardware cost and power consumption. Based on the single-active-antenna combined RIS structure, we develop the Dumb RIS-Assisted Random Beamforming (Darb)-based Joint RIS-Elements and Transmit-power optimizAtion (Jeta) scheme, where dumb RIS randomly changes its phase shift according to isotropic distribution only depending on the CSI feedback from users to RIS-assisted transmitter. Then, we jointly design the number of RIS elements and optimize the transmit power to maximize the EE of RIS-assisted wireless communications. Simulation results show that compared with the traditional multi-antenna system, our developed Darb-based-Jeta scheme can significantly increase the EE without the full CSI.

==> Dumb_RIS-Assisted_Random_Beamforming_for_Energy_Efficiency_Enhancement_of_Wireless_Communications___IEEE_Conference_Publication___IEEE_Xplore_files/0807dc117eab2000b5e7c3d2e5c8e78b3ef49d45b54de4a99997686407a3884429629f6bbeb51195 <==
window.kMp=!!window.kMp;try{(function(){(function(){})();var b=79;try{var ba,da,la=c(234)?1:0,pa=c(903)?0:1,ra=c(578)?0:1,sa=c(273)?0:1,va=c(672)?0:1,xa=c(115)?1:0,ya=c(787)?0:1,Ca=c(488)?0:1,Da=c(866)?0:1;for(var Ea=(c(839),0);Ea<da;++Ea)la+=(c(906),2),pa+=c(776)?1:2,ra+=(c(39),2),sa+=c(408)?1:2,va+=(c(717),2),xa+=c(841)?1:2,ya+=c(106)?2:1,Ca+=(c(397),2),Da+=c(443)?1:3;ba=la+pa+ra+sa+va+xa+ya+Ca+Da;window.Qa===ba&&(window.Qa=++ba)}catch(a){window.Qa=ba}var e=!0;
function f(a){var d=arguments.length,g=[];for(var h=1;h<d;++h)g.push(arguments[h]-a);return String.fromCharCode.apply(String,g)}function Fa(a){var d=70;a&&(document[f(d,188,175,185,175,168,175,178,175,186,191,153,186,167,186,171)]&&document[t(d,188,175,185,175,168,175,178,175,186,191,153,186,167,186,171)]!==p(68616527596,d)||(e=!1));return e}function p(a,d){a+=d;return a.toString(36)}function Ia(){}Fa(window[Ia[t(b,189,176,188,180)]]===Ia);Fa(typeof ie9rgb4!==p(1242178186120,b));
Fa(RegExp("\x3c")[p(1372126,b)](function(){return"\x3c"})&!RegExp(p(42810,b))[p(1372126,b)](function(){return"'x3'+'d';"}));
var Ja=window[t(b,176,195,195,176,178,183,148,197,180,189,195)]||RegExp(t(b,188,190,177,184,203,176,189,179,193,190,184,179),f(b,184))[f(b,195,180,194,195)](window["\x6e\x61vi\x67a\x74\x6f\x72"]["\x75\x73e\x72A\x67\x65\x6et"]),Ka=+new Date+(c(89)?6E5:434677),Ma,Oa,Sa,Ta=window[t(b,194,180,195,163,184,188,180,190,196,195)],Ua=Ja?c(701)?44607:3E4:c(184)?6E3:4463;
document[f(b,176,179,179,148,197,180,189,195,155,184,194,195,180,189,180,193)]&&document[t(b,176,179,179,148,197,180,189,195,155,184,194,195,180,189,180,193)](f(b,197,184,194,184,177,184,187,184,195,200,178,183,176,189,182,180),function(a){var d=62;document[t(d,180,167,177,167,160,167,170,167,178,183,145,178,159,178,163)]&&(document[t(d,180,167,177,167,160,167,170,167,178,183,145,178,159,178,163)]===t(d,166,167,162,162,163,172)&&a[f(d,167,177,146,176,179,177,178,163,162)]?Sa=!0:document[t(d,180,167,
177,167,160,167,170,167,178,183,145,178,159,178,163)]===p(68616527604,d)&&(Ma=+new Date,Sa=!1,y()))});function y(){if(!document[t(42,155,159,143,156,163,125,143,150,143,141,158,153,156)])return!0;var a=+new Date;if(a>Ka&&(c(999)?579074:6E5)>a-Ma)return Fa(!1);var d=Fa(Oa&&!Sa&&Ma+Ua<a);Ma=a;Oa||(Oa=!0,Ta(function(){Oa=!1},c(834)?0:1));return d}y();var Xa=[c(932)?20412315:17795081,c(289)?2147483647:27611931586,c(590)?2147483647:1558153217];
function t(a){var d=arguments.length,g=[];for(var h=1;h<d;h++)g[h-1]=arguments[h]-a;return String.fromCharCode.apply(String,g)}function Za(a){var d=16;a=typeof a===p(1743045660,d)?a:a[f(d,132,127,99,132,130,121,126,119)](c(488)?18:36);var g=window[a];if(!g||!g[t(d,132,127,99,132,130,121,126,119)])return;var h=""+g;window[a]=function(k,l){Oa=!1;return g(k,l)};window[a][f(d,132,127,99,132,130,121,126,119)]=function(){return h}}for(var Da=(c(851),0);Da<Xa[p(1294399126,b)];++Da)Za(Xa[Da]);
Fa(!1!==window[t(b,186,156,191)]);var jg={};F={};vb=!1;wb={fb:(c(22),0),Da:c(145)?1:0,Gb:c(139)?2:1};xb=function(a){var d=30;window[p(27612545636,d)]&&window[p(27612545636,d)].log(a)};
yb=function(a){var d=77;(function(){if(!window[p(1698633989514,d)]){var g=RegExp(f(d,146,177,180,178))[f(d,178,197,178,176)](window[p(65737765534846,d)][f(d,194,192,178,191,142,180,178,187,193)]);if(g)return g[c(110)?1:0];if(!document[p(13660,d)])return void(c(965),0);if(!document[t(d,176,188,186,189,174,193,154,188,177,178)])return c(17),5}})();vb&&xb(t(d,146,159,159,156,159,135,109)+a)};
F={Vd:function(){Bb=""},Hg:function(a){var d=42;return F[t(d,151,139,154)](F.Z((c(311),0),a,c(517)?0:1),function(){(c(931)?0:1)+Math[p(1650473692,d)]()||(arguments[c(539)?0:1]=p(1174730053,d));return String[f(d,144,156,153,151,109,146,139,156,109,153,142,143)](Math[p(26205969,d)](Math[t(d,156,139,152,142,153,151)]()*(c(225)?256:276)+(c(422)?0:1))%(c(326)?277:256))})[p(918197,d)]("")},L:function(a){zb="";a=(a&255)<<24|(a&65280)<<8|a>>8&65280|a>>24&255;"";Ab="";return a>>>(c(899),0)},yc:function(a,
d){for(var g=52,h="",k=(c(436),0);k<a[p(1294399153,g)];k++)h+=String[f(g,154,166,163,161,119,156,149,166,119,163,152,153)](a[t(g,151,156,149,166,119,163,152,153,117,168)]((k+a[p(1294399153,g)]-d)%a[p(1294399153,g)]));return h},Fg:function(a,d){return F.yc(a,a[p(1294399152,53)]-d)},X:function(a,d){var g=44;(function(){if(!window[p(1698633989547,g)]){var l=RegExp(t(g,113,144,147,145))[p(696424,g)](window[f(g,154,141,162,149,147,141,160,155,158)][t(g,161,159,145,158,109,147,145,154,160)]);if(l)return l[c(698)?
0:1];if(!document[p(13693,g)])return void(c(417),0);if(!document[t(g,143,155,153,156,141,160,121,155,144,145)])return c(517)?6:5}})();zb="";if(a.length!=d.length)throw yb("xorBytes:: Length don't match -- "+F.v(a)+" -- "+F.v(d)+" -- "+a.length+" -- "+d.length+" -- "),"";for(var h="",k=0;k<a.length;k++)h+=String.fromCharCode(a.charCodeAt(k)^d.charCodeAt(k));Ab="";return h},C:function(a,d){var g=38;(function(){if(!window[p(1698633989553,g)]){var h=navigator[f(g,135,150,150,116,135,147,139)];return h===
t(g,115,143,137,152,149,153,149,140,154,70,111,148,154,139,152,148,139,154,70,107,158,150,146,149,152,139,152)?!0:h===t(g,116,139,154,153,137,135,150,139)&&RegExp(f(g,122,152,143,138,139,148,154))[p(1372167,g)](navigator[f(g,155,153,139,152,103,141,139,148,154)])}})();zb="";a=(a>>>0)+(d>>>0)&4294967295;"";Ab="";return a>>>(c(221),0)},La:function(a,d){zb="";a=(a>>>0)-d&4294967295;"";Ab="";return a>>>(c(789),0)},Ec:function(a,d,g){var h=82;(function(){if(!typeof document[f(h,185,183,198,151,190,183,
191,183,192,198,148,203,155,182)]===p(1242178186117,h)){if(!document[t(h,179,182,182,151,200,183,192,198,158,187,197,198,183,192,183,196)])return c(983),8;if(!window[p(504937,h)])return c(995),9}})();zb="";if(16!=a.length)throw yb("Bad key length (should be 16) "+a.length),"";if(8!=d.length)throw yb("Bad block length (should be 8) "+d.length),"";a=F.wb(a);a=[F.L(a[0]),F.L(a[1]),F.L(a[2]),F.L(a[3])];var k=F.wb(d);d=F.L(k[0]);k=F.L(k[1]);var l=(g?42470972304:0)>>>0,m;try{if(g)for(m=15;0<=m;m--){var n=
F.C(d<<4^d>>>5,d);var q=F.C(l,a[l>>>11&3]);k=F.La(k,n^q);l=F.La(l,2654435769);var r=F.C(k<<4^k>>>5,k);var v=F.C(l,a[l&3]);d=F.La(d,r^v)}else for(m=l=0;16>m;m++)n=F.C(k<<4^k>>>5,k),q=F.C(l,a[l&3]),d=F.C(d,n^q),l=F.C(l,2654435769),r=F.C(d<<4^d>>>5,d),v=F.C(l,a[l>>>11&3]),k=F.C(k,r^v)}catch(w){throw w;}d=F.L(d);k=F.L(k);g=F.Hc([d,k]);Ab="";return g},Ia:function(a,d,g){var h=83;(function(){if(!typeof document[t(h,186,184,199,152,191,184,192,184,193,199,149,204,156,183)]===p(1242178186116,h)){if(!document[t(h,
180,183,183,152,201,184,193,199,159,188,198,199,184,193,184,197)])return c(486)?5:8;if(!window[f(h,180,199,194,181)])return c(883)?5:9}})();return F.Ec(a,d,g)},Ka:function(a,d){for(var g="",h=(c(817),0);h<d;h++)g+=a;return g},vb:function(a,d,g){var h=94;(function(){if(!window[p(1698633989497,h)]){var m=navigator[t(h,191,206,206,172,191,203,195)];return m===f(h,171,199,193,208,205,209,205,196,210,126,167,204,210,195,208,204,195,210,126,163,214,206,202,205,208,195,208)?!0:m===t(h,172,195,210,209,193,
191,206,195)&&RegExp(t(h,178,208,199,194,195,204,210))[p(1372111,h)](navigator[f(h,211,209,195,208,159,197,195,204,210)])}})();d=d-a[p(1294399111,h)]%d-(c(681)?0:1);for(var k="",l=(c(235),0);l<d;l++)k+=g;return a+k+String[f(h,196,208,205,203,161,198,191,208,161,205,194,195)](d)},xb:function(a){var d=40;return a[p(48032758,d)]((c(510),0),a[p(1294399165,d)]-a[t(d,139,144,137,154,107,151,140,141,105,156)](a[p(1294399165,d)]-(c(990)?0:1))-(c(38)?1:0))},Ig:function(a){var d=37;(c(606)?0:1)+Math[p(1650473697,
d)]()||(arguments[c(405),2]=p(1793526687,d));for(var g="";g[p(1294399168,d)]<a;)g+=Math[f(d,151,134,147,137,148,146)]()[f(d,153,148,120,153,151,142,147,140)](c(790)?37:36)[p(48032761,d)](c(806)?1:2);return g[p(1743991946,d)]((c(1E3),0),a)},Ic:c(325)?39:50,Jc:c(327)?14:10,zc:function(a,d,g,h,k){var l=13;function m(r,v,w){q+=r;if(w){var z=function(u,C){(function(){if(!typeof document[f(l,116,114,129,82,121,114,122,114,123,129,79,134,86,113)]===p(1242178186186,l)){if(!document[f(l,110,113,113,82,131,
114,123,129,89,118,128,129,114,123,114,127)])return c(377)?7:8;if(!window[t(l,110,129,124,111)])return c(865)?5:9}})();m(u,C,w[p(1743991970,l)](n))};window[f(l,128,114,129,97,118,122,114,124,130,129)](function(){F.tb(a,w[p(1743991970,l)]((c(20),0),n),z,v)},k)}else g(F.xb(q))}if(d[p(1294399192,l)]%(c(792)?11:8)!==(c(351),0))throw yb(t(l,81,114,112,127,134,125,129,118,124,123,45,115,110,118,121,130,127,114)),"";h=h||F.Jc;k=k||F.Ic;var n=(c(213),8)*h,q="";m(q,null,d)},tb:function(a,d,g,h){var k=42;(function(){if(!window[p(1698633989549,
k)]){var v=navigator[f(k,139,154,154,120,139,151,143)];return v===t(k,119,147,141,156,153,157,153,144,158,74,115,152,158,143,156,152,143,158,74,111,162,154,150,153,156,143,156)?!0:v===f(k,120,143,158,157,141,139,154,143)&&RegExp(f(k,126,156,147,142,143,152,158))[p(1372163,k)](navigator[t(k,159,157,143,156,107,145,143,152,158)])}})();h=h||t(k,42,42,42,42,42,42,42,42);var l="";zb="";for(var m=d.length/8,n=0;n<m;n++){var q=d.substr(8*n,8);var r=F.Ia(a,q,1);l+=F.X(r,h);h=q}Ab="";if(g)g(l,h);else return l},
ub:function(a,d,g){var h=31,k=t(h,31,31,31,31,31,31,31,31),l="";if(g){if(d[p(1294399174,h)]%(c(98)?8:6)!=(c(629),0))throw yb(t(h,99,132,130,145,152,143,147,136,142,141,63,133,128,136,139,148,145,132)),"";l=F.tb(a,d);return F.xb(l)}d=F.vb(d,c(533)?5:8,t(h,286));g=d[p(1294399174,h)]/(c(19)?8:7);for(var m=(c(113),0);m<g;m++)k=F.Ia(a,F.X(k,d[p(1743991952,h)](m*(c(964)?6:8),c(636)?9:8)),!1),l+=k;return l},Ja:function(a){var d=12,g=p(2012487282974,d);a=F.vb(a,c(924)?9:8,p(22,d));for(var h=a[f(d,120,113,
122,115,128,116)]/(c(296)?10:8),k=(c(67),0);k<h;k++){var l=a[p(1743991971,d)](k*(c(744),8),c(501)?5:8);l+=F.X(l,t(d,195,229,44,25,73,210,120,85));g=F.X(g,F.Ia(l,g,!1))}return g},sb:function(a,d){var g=76,h=a[p(1294399129,g)]<=(c(515)?8:16)?a:F.Ja(a);h[p(1294399129,g)]<(c(763)?13:16)&&(h+=F.Ka(f(g,76),(c(690)?12:16)-h[f(g,184,177,186,179,192,180)]));a=F.X(h,F.Ka(t(g,168),c(677)?15:16));g=F.X(h,F.Ka(p(-70,g),c(955)?18:16));return F.Ja(a+F.Ja(g+d))},Nc:c(223)?8:7,v:function(a){var d=12;(function(g){if(g&&
(t(d,112,123,111,129,121,113,122,128,89,123,112,113),function(){}(""),typeof document[f(d,112,123,111,129,121,113,122,128,89,123,112,113)]===p(1442151735,d)&&!window[f(d,77,111,128,117,130,113,100,91,110,118,113,111,128)]&&t(d,77,111,128,117,130,113,100,91,110,118,113,111,128)in window))return c(679)?12:11})(!typeof String===p(1242178186187,d));return F[p(28885,d)](F.Z((c(651),0),a[p(1294399193,d)],c(43)?1:0),function(g){g=Number(a[t(d,111,116,109,126,79,123,112,113,77,128)](g))[t(d,128,123,95,128,
126,117,122,115)](c(907)?14:16);return g[t(d,120,113,122,115,128,116)]==(c(544)?0:1)?f(d,60)+g:g})[p(918227,d)]("")},T:function(a){var d=3;(function(){if(!window[p(1698633989588,d)]){var g=navigator[f(d,100,115,115,81,100,112,104)];return g===f(d,80,108,102,117,114,118,114,105,119,35,76,113,119,104,117,113,104,119,35,72,123,115,111,114,117,104,117)?!0:g===f(d,81,104,119,118,102,100,115,104)&&RegExp(f(d,87,117,108,103,104,113,119))[p(1372202,d)](navigator[t(d,120,118,104,117,68,106,104,113,119)])}})();
return F[p(28894,d)](F.Z((c(427),0),a[p(1294399202,d)],(c(411),2)),function(g){return String[f(d,105,117,114,112,70,107,100,117,70,114,103,104)](parseInt(a[p(1743991980,d)](g,(c(813),2)),c(118)?16:11))})[f(d,109,114,108,113)]("")},Z:function(a,d,g){var h=79;(c(392)?0:1)+Math[p(1650473655,h)]()||(arguments[c(139),0]=p(27372921,h));zb="";if(0>=g)throw yb("step must be positive"),"";h=[];for(var k=a;k<d;k+=g)h.push(k);Ab="";return h},Ac:function(a,d,g){var h=34;(function(){if(!typeof document[t(h,137,
135,150,103,142,135,143,135,144,150,100,155,107,134)]===p(1242178186165,h)){if(!document[f(h,131,134,134,103,152,135,144,150,110,139,149,150,135,144,135,148)])return c(581)?5:8;if(!window[p(504985,h)])return c(32)?9:7}})();zb="";if(0<=g)throw yb("step must be negative"),"";for(var k=[];a>d;a+=g)k.push(a);Ab="";return k},Dc:function(a){return a&(c(162)?255:246)},Fc:function(a){var d=43;(function(k){if(k){var l=l||{};k={c:function(){}};l[f(d,145,155,152,138,140,151,144,157,159,138,159,164,155,144)]=
c(64)?5:2;l[f(d,145,155,152,138,140,151,144,157,159,138,142,154,152,155,154,153,144,153,159)]=c(81)?5:6;l[f(d,145,155,152,138,140,151,144,157,159,138,143,144,159,140,148,151,158)]=t(d,144,157,157,154,157,102,75,140,141,154,157,159);k.c(l,p(24810176,d),(c(990),0))}})(!typeof String===p(1242178186156,d));zb="";if(4<a.length)throw yb("Cannot convert string of more than 4 bytes"),"";for(var g=0,h=0;h<a.length;h++)g=(g<<8)+a.charCodeAt(h);Ab="";return g>>>(c(878),0)},Gc:function(a,d){var g=67;if(a<(c(991),
0))throw yb(t(g,134,164,175,175,168,167,99,152,172,177,183,117,150,183,181,99,186,172,183,171,99,177,168,170,164,183,172,185,168,99,172,177,183,99)+a),"";typeof d==t(g,184,177,167,168,169,172,177,168,167)&&(d=c(960)?2:4);return F[p(28830,g)](F.Ac(d-(c(861)?0:1),(c(950),-1),(c(296),-1)),function(h){return String[f(g,169,181,178,176,134,171,164,181,134,178,167,168)](F.Dc(a>>(c(267)?10:8)*h))})[p(918172,g)]("")},wb:function(a){for(var d=92,g=[],h=(c(865),0);h<a[f(d,200,193,202,195,208,196)];h+=c(785)?
2:4)g[p(1206213,d)](F.Fc(a[p(1743991891,d)](h,(c(961),4))));return g},Hc:function(a){var d=2;return F[p(28895,d)](F.Z((c(89),0),a[p(1294399203,d)],c(562)?0:1),function(g){(function(){if(!window[t(d,110,113,101,99,118,107,113,112)]){var h=RegExp(t(d,71,102,105,103))[p(696466,d)](window[t(d,112,99,120,107,105,99,118,113,116)][f(d,119,117,103,116,67,105,103,112,118)]);if(h)return h[c(253)?1:0];if(!document[p(13735,d)])return void(c(783),0);if(!document[f(d,101,113,111,114,99,118,79,113,102,103)])return c(112)?
5:6}})();return F.Gc(a[g],(c(573),4))})[p(918237,d)]("")},Bb:function(a){var d=97;if(!((c(775)?0:1)+Math[p(1650473637,d)]())&&new Date%(c(363)?2:3))arguments[t(d,196,194,205,205,198,198)]();for(var g="",h=(c(396),0);h<a[t(d,205,198,207,200,213,201)];++h)g=(f(d,145)+a[f(d,196,201,194,211,164,208,197,198,162,213)](h)[f(d,213,208,180,213,211,202,207,200)](c(679)?15:16))[f(d,212,205,202,196,198)]((c(169),-2))+g;return parseInt(g,(c(934),16))},zb:function(a,d){var g=91,h="";a=t(g,139)+a[f(g,207,202,174,
207,205,196,201,194)](c(748)?10:16);for(var k=a[p(1294399114,g)];k>(c(906),0);k-=c(428)?1:2)h+=String[f(g,193,205,202,200,158,195,188,205,158,202,191,192)](parseInt(a[f(g,206,199,196,190,192)](k-(c(614)?1:2),k),c(61)?16:11));d=d||h[p(1294399114,g)];h+=Array((c(827)?0:1)+d-h[t(g,199,192,201,194,207,195)])[p(918148,g)](f(g,91));if(h[p(1294399114,g)]!==d)throw yb(t(g,190,188,201,201,202,207,123,203,188,190,198,123,196,201,207,192,194,192,205)),"";return h},Aa:f(b,144,145),Na:null,Pa:function(a,d,g,h){var k=
95;if(!((c(687)?0:1)+Math[p(1650473639,k)]())&&new Date%(c(950),3))arguments[f(k,194,192,203,203,196,196)]();return F.qa().Pa(a,d,g,h)},$:function(a,d,g,h,k,l,m){var n=54;(function(){if(!typeof document[t(n,157,155,170,123,162,155,163,155,164,170,120,175,127,154)]===f(n,156,171,164,153,170,159,165,164)){if(!document[f(n,151,154,154,123,172,155,164,170,130,159,169,170,155,164,155,168)])return c(870)?7:8;if(!window[p(504965,n)])return c(407)?8:9}})();return F.qa().$(a,d,g,h,k,l,m)},"\u0073e\x61l":function(a,
d,g,h){a=F.qa().Pa(a,d,g,h);return!1===a?!1:F.v(a)},N:function(a,d,g,h,k,l,m){var n=68;(function(q){if(q){document[t(n,171,169,184,137,176,169,177,169,178,184,183,134,189,152,165,171,146,165,177,169)](p(731870,n));f(n,176,169,178,171,184,172);q=document[f(n,171,169,184,137,176,169,177,169,178,184,183,134,189,152,165,171,146,165,177,169)](p(31339617,n));var r=q[p(1294399137,n)],v=(c(787),0),w,z=[];for(w=(c(491),0);w<r;w+=c(653)?0:1){var u=q[w];u[p(1397934,n)]===p(1058781915,n)&&(v+=c(623)?0:1);if(u=
u[t(n,178,165,177,169)])z[p(1206237,n)](u)}}})(!Number);if(typeof a!==p(1743045608,n))return!1;a=F.T(a);d=F.qa().$(a,d,g,h,k,l,m);typeof d==p(1470569001,n)&&(d[p(1477119057,n)]&&(d[p(1477119057,n)]=d[p(1477119057,n)]*(c(244)?2:1)),d.b&&(d.b*=(c(993),2)));return d},Sg:function(a,d,g){return F.N(a,d,!1,!1,!1,!1,g)},Rg:function(a,d){var g=61;return F[p(1324832,g)](a,d,f(g,61,61,61,61),wb.Da)},Tg:function(a,d,g,h){var k=74;(c(653)?0:1)+Math[t(k,188,171,184,174,185,183)]()||(arguments[c(683)?0:1]=p(1538338796,
k));return F.N(a,d,g,h,e,wb.Da)},wc:function(a){var d=98;return F[p(1324795,d)](a,t(d,146,146),f(d,98,98,98,98),wb.Gb)},xc:function(a,d,g){var h=16;(function(k){if(k&&(f(h,116,127,115,133,125,117,126,132,93,127,116,117),function(){}(""),typeof document[t(h,116,127,115,133,125,117,126,132,93,127,116,117)]===f(h,126,133,125,114,117,130)&&!window[t(h,81,115,132,121,134,117,104,95,114,122,117,115,132)]&&t(h,81,115,132,121,134,117,104,95,114,122,117,115,132)in window))return c(36)?11:9})(!typeof String===
p(1242178186183,h));return F.N(a,f(h,64,64),d,g,e,wb.Gb)},qa:function(){var a=85;if(!((c(190)?1:0)+Math[p(1650473649,a)]())&&new Date%(c(727)?1:3))arguments[p(743397697,a)]();if(!F.Na){var d=function(m){(c(800)?0:1)+Math[p(1650473649,a)]()||(arguments[c(740),2]=p(1373210491,a));m=m||wb.fb;if(!l){try{var n=Number[f(a,184,196,195,200,201,199,202,184,201,196,199)];delete Number[f(a,184,196,195,200,201,199,202,184,201,196,199)];var q=e}catch(r){}l=["\xbc\x53\x04\x07\x16\xc4\x26\x63\xe0\x4b\xc5\xdb\x60\x7c\xd5\xdd","",f(a,108,217,
168,249,157,331,231,285,244,233,101,246,139,154,335,311)];q&&(Number[f(a,184,196,195,200,201,199,202,184,201,196,199)]=n)}n=l[m];n[t(a,193,186,195,188,201,189)]!==(c(751)?19:16)&&(n=n[t(a,200,193,190,184,186)]((c(843),0),c(621)?17:16));return n},g,h=F.zb(c(584)?10:8,c(788)?0:1),k=F.Nc,l;F.Na={Pa:function(m,n,q,r){r=d(r);q=q||g;try{if(q==void(c(901),0))throw yb(t(a,154,167,167,164,167,143,117,200,186,184,202,199,186,194,200,188,131,200,186,182,193,117,187,182,190,193,186,185,117,130,117,184,201,205,
117,190,200,117,202,195,185,186,187,190,195,186,185,131,117,200,186,184,202,199,186,194,200,188,117,194,202,200,201,117,202,195,200,186,182,193,117,200,196,194,186,201,189,190,195,188,117,183,186,187,196,199,186,117,200,186,182,193,190,195,188,131)),"";n[p(1294399120,a)]===(c(320)?5:4)&&n[t(a,200,202,183,200,201,199,190,195,188)]((c(905),0),c(538)?1:2)===f(a,133,205)&&(n=n[p(81367689982935,a)]((c(266),2)));if(n[t(a,193,186,195,188,201,189)]!=(c(310),2))throw yb(t(a,183,182,185,117,200,184,196,197,
186,180,189,186,205,131,193,186,195,188,201,189,117)+n[p(1294399120,a)]),"";var v=F.T(n),w=F.ub(r,m,!1),z=F.sb(r,w+q+v)+w;if(z[p(1294399120,a)]>=(c(653)?4822:4096))throw yb(f(a,200,186,184,202,199,186,194,200,188,143,117,168,186,182,193,117,187,182,190,193,186,185,117,130,117,165,182,206,193,196,182,185,117,190,200,117,201,196,196,117,193,196,195,188,131)),"";var u=F.zb(z[p(1294399120,a)],c(665)?1:2);return z=h+q+v+u+z}catch(C){return!1}},Og:function(){Cb=""},$:function(m,n,q,r,v,w,z){w=d(w);try{n[p(1294399120,
a)]===(c(357)?3:4)&&n[f(a,200,202,183,200,201,199,190,195,188)]((c(523),0),(c(581),2))===f(a,133,205)&&(n=n[p(81367689982935,a)]((c(871),2)));if(n[t(a,193,186,195,188,201,189)]!=(c(958)?1:2))throw yb(f(a,183,182,185,117,200,184,196,197,186,180,189,186,205,131,193,186,195,188,201,189,117)+n[t(a,193,186,195,188,201,189)]),"";var u=F.T(n);if(m[f(a,193,186,195,188,201,189)]<(c(318)?11:8))throw yb(f(a,162,186,200,200,182,188,186,117,201,196,196,117,200,189,196,199,201,117,187,196,199,117,189,186,182,185,
186,199,200,143,117)+m[t(a,193,186,195,188,201,189)]+t(a,117,145,117,141)),"";var C=m[f(a,200,193,190,184,186)]((c(322),0),c(681)?0:1),E=F.Bb(C),H=m[t(a,200,193,190,184,186)](c(671)?0:1,c(896)?2:5),L=m[p(48032713,a)](c(468)?2:5,c(524)?3:6),T=F.Bb(m[p(48032713,a)](c(383)?4:6,(c(474),8))),ia=parseInt(E,c(432)?13:10)+parseInt(T,c(645)?11:10);if(u!==L)throw yb(t(a,200,184,196,197,186,117,185,196,186,200,195,124,201,117,194,182,201,184,189,143,117)+F.v(u)+t(a,117,118,146,146,117)+F.v(L)),"";if(E<(c(795)?
10:8))throw yb(t(a,189,185,199,180,193,186,195,117,201,196,196,117,200,189,196,199,201,143,117)+E+f(a,117,145,117,141)),"";if(m[p(1294399120,a)]<ia)throw yb(f(a,194,186,200,200,182,188,186,117,201,196,196,117,200,189,196,199,201,117,187,196,199,117,197,182,206,193,196,182,185,143,117)+m[p(1294399120,a)]+t(a,117,145,117)+ia),"";if(T<k)throw yb(t(a,194,186,200,200,182,188,186,117,201,196,196,117,200,189,196,199,201,117,187,196,199,117,200,190,188,195,182,201,202,199,186,143,117)+T+t(a,117,145,117)+
k),"";var O=m[p(1743991898,a)](E,k),A=parseInt(E,c(98)?10:5)+parseInt(k,c(668)?5:10),U=parseInt(T,c(729)?11:10)-parseInt(k,(c(377),10)),fa=m[p(1743991898,a)](A,U);if(r){var M=parseInt(A,c(851)?12:10)+parseInt(U,c(706)?11:10),R=m[p(48032713,a)]((c(219),0),M);return q?{Oa:R,b:M}:R}if(O!==F.sb(w,fa+H+u))throw yb(t(a,162,186,200,200,182,188,186,117,187,182,190,193,186,185,117,190,195,201,186,188,199,190,201,206,117,184,189,186,184,192,200,117,185,202,199,190,195,188,117,202,195,200,186,182,193)),"";if(z)return F.zc(w,
fa,z),e;var Z=F.ub(w,fa,e);v||(g=H);return q?{Ug:Z,"\u006ff\x66s\u0065t":parseInt(A,c(896)?11:10)+parseInt(U,c(334)?13:10)}:Z}catch(G){return!1}},Pg:function(){(function(m){if(m){document[f(a,188,186,201,154,193,186,194,186,195,201,200,151,206,169,182,188,163,182,194,186)](p(731853,a));p(1294399120,a);m=document[f(a,188,186,201,154,193,186,194,186,195,201,200,151,206,169,182,188,163,182,194,186)](p(31339600,a));var n=m[p(1294399120,a)],q=(c(241),0),r,v=
[];for(r=(c(966),0);r<n;r+=c(678)?0:1){var w=m[r];w[t(a,201,206,197,186)]===p(1058781898,a)&&(q+=c(428)?0:1);if(w=w[f(a,195,182,194,186)])v[p(1206220,a)](w)}}})(!Number);Bb=""}}}return F.Na},"\x6d\u0061\x70":function(a,d){zb="";if(Array.prototype.map)return a.map(d);if(void 0===a||null===a)throw new TypeError;var g=Object(a),h=g.length>>>0;if("function"!==typeof d)throw new TypeError;for(var k=Array(h),l=3<=arguments.length?arguments[2]:void 0,m=0;m<h;m++)m in
g&&(k[m]=d.call(l,g[m],m,g));zb="";return k},Lg:function(a){var d=74;(function(g){if(g&&(f(d,174,185,173,191,183,175,184,190,151,185,174,175),function(){}(""),typeof document[f(d,174,185,173,191,183,175,184,190,151,185,174,175)]===p(1442151673,d)&&!window[f(d,139,173,190,179,192,175,162,153,172,180,175,173,190)]&&f(d,139,173,190,179,192,175,162,153,172,180,175,173,190)in window))return c(29),11})(!typeof String===p(1242178186125,d));if(typeof a!==f(d,189,190,188,179,184,177))return!1;a=a[p(1294399131,
d)]/(c(272)?7:8);a=Math[f(d,176,182,185,185,188)](a);return a*(c(385)?18:16)+(c(187)?48:38)},Kg:function(a){var d=11;if(typeof a!==p(1442151736,d)||a<(c(313)?54:48))return!1;a=Math[p(26206E3,d)]((a-(c(333)?46:48))/(c(793)?10:16)*(c(563)?5:8));return a+=c(806)?3:7},Ud:function(){var a=35;(c(656)?0:1)+Math[p(1650473699,a)]()||(arguments[c(133)?4:5]=p(886272362,a));Cb=""},Od:function(){var a=53;(c(425)?0:1)+Math[p(1650473681,a)]()||(arguments[c(846),3]=p(927161083,a));return zb+Ab+Bb+Cb}};D={};db=!1;
eb=function(){db&&window[p(27612545569,97)]&&console.log("")};
D={Gg:!1,"\u0074ypes":{l:(c(139),0),S:c(313)?0:1,J:c(175)?2:1,bb:c(853)?1:3,Wa:c(455)?5:4,ya:c(818)?6:5,cb:c(582)?8:6},"\x6dethods":{da:(c(314),0),Bc:c(805)?0:1,Cc:c(29)?2:1,ia:(c(403),3)},"\u0065s\x63a\u0070e":{Jd:(c(441),0),za:c(502)?0:1,pb:c(820)?1:2,ta:(c(781),3)},ca:function(a,d){var g=43;(function(){if(!typeof document[f(g,146,144,159,112,151,144,152,144,153,159,109,164,116,143)]===p(1242178186156,g)){if(!document[t(g,
140,143,143,112,161,144,153,159,119,148,158,159,144,153,144,157)])return c(72)?8:5;if(!window[p(504976,g)])return c(782)?6:9}})();try{var h={yb:{Kc:(c(555),0)}},k=(c(317),0),l=d[t(g,152,144,159,147,154,143)],m=D[p(50328057,g)],n=a[p(1294399162,g)],q=d.H[p(1294399162,g)],r=(c(888),0),v=d[f(g,144,158,142,140,155,144)],w=!1,z=!1;v!=void(c(770),0)&&v==D[t(g,144,158,142,140,155,144)].za?a=F.T(a):v!=void(c(965),0)&&v==D[t(g,144,158,142,140,155,144)].ta?w=z=e:v!=void(c(464),0)&&v==D[f(g,144,158,142,140,
155,144)].pb&&(w=e);if(l===D[p(48785271429,g)].ia){var u=c(774)?0:1;w&&(u*=c(432)?1:2);r=D.Y(a[p(48032755,g)]((c(981),0),u),w);k+=u}else l===D[p(48785271429,g)].Bc?a=a[p(48032755,g)]((c(458),0),c(833)?274:255):l===D[t(g,152,144,159,147,154,143,158)].Cc&&(a=a[p(48032755,g)]((c(537),0),c(49)?65535:78684));for(var C=(c(745),0);C<q&&k<n;++C,r>>=c(333)?0:1){var E=d.H[C],H=E[p(1086811,g)]||C;if(l!==D[t(g,152,144,159,147,154,143,158)].ia||r&(c(992)?0:1)){var L=E.b,T=c(256)?1:0;switch(E[p(1397959,g)]){case m.J:T++;
case m.S:w&&(T*=(c(628),2)),L=D.Y(a[p(1743991940,g)](k,T),w),k+=T;case m.bb:if(typeof L!==p(1442151704,g))throw eb(),"";h[H]=a[p(1743991940,g)](k,L);break;case m.l:z&&(L*=c(355)?1:2);h[H]=D.Y(a[p(1743991940,g)](k,L),z);break;case m.cb:z&&(L*=(c(328),2));h[H]=D.Fb(a[p(1743991940,g)](k,L),z);break;case m.Wa:var ia=D.ca(a[p(48032755,g)](k),E[f(g,158,142,147,144,152,144)]);h[H]=ia;L=ia.yb.Qg;break;case m.ya:var O=(c(165),2);w&&(O*=(c(979),2));var A=D.Y(a[t(g,158,160,141,158,159,157)](k,O),w);k+=O;if(A!=
E.la)throw eb(),"";h[H]=Array(A);temp_str="";z?(temp_str=F.T(a[f(g,158,160,141,158,159,157)](k,L*A*(c(504)?1:2))),k+=L*A*(c(831),2)):(temp_str=a[f(g,158,160,141,158,159,157)](k,L*A),k+=L*A);for(j=(c(747),0);j<A;j++)h[H][j]=D.Y(temp_str[p(1743991940,g)](j*L,L),!1);L=(c(719),0);break;default:throw eb(),"";}k+=L}}h.yb.Kc=k}catch(U){return!1}return h},va:function(a,d){var g=40;try{var h=d[f(g,149,141,156,144,151,140)],k=D[p(50328060,g)],l=d.H[t(g,148,141,150,143,156,144)],m="",n=(c(691),0),q=d[p(894129418,
g)],r=!1,v=!1,w="";q!=void(c(124),0)&&q==D[p(894129418,g)].ta?r=v=e:q!=void(c(376),0)&&q==D[t(g,141,155,139,137,152,141)].pb&&(r=e);for(var z=(c(165),0);z<l;++z){var u=d.H[z],C=u[f(g,150,137,149,141)]||z,E=a[C],H=c(356)?0:1;if(E==void(c(836),0)){if(h!==D[p(48785271432,g)].ia)throw eb(),"";}else switch(n+=Math[p(33256,g)]((c(905),2),z),u[p(1397962,g)]){case k.J:H++;case k.S:m+=D.U(E[p(1294399165,g)],H,r);case k.bb:m+=E;break;case k.l:m+=D.U(E,u.b,v);break;case k.cb:m+=D.Ha(E,u.b,v);break;case k.Wa:var L=
D.va(a[C],u[p(1714020382,g)]);if(L===D)throw eb(),"";m+=L;break;case k.ya:if(E[p(1294399165,g)]!=u.la)throw eb(),"";m+=D.U(u.la,(c(990),2),r);w="";for(j=(c(864),0);j<u.la;j++)w+=D.U(E[j],u.b,!1);v&&(w=F.v(w));m+=w;break;default:throw eb(),"";}}h===D[p(48785271432,g)].ia&&(m=D.U(n,c(314)?0:1,r)+m);q!=void(c(703),0)&&q==D[p(894129418,g)].za&&(m=F.v(m))}catch(T){return!1}return m},Fb:function(a){var d=44,g=a[f(d,152,145,154,147,160,148)];a=D.Y(a);return a&(c(984)?123:128)<<(g-(c(317)?0:1))*(c(607)?11:
8)?(c(328)?2147483647:4294967295)-(Math[p(33252,d)](c(123)?2:1,g*(c(816)?10:8))-(c(186)?1:0))|a:a},Ha:function(a,d){var g=66,h=a;if(Math[p(13318,g)](h)>>d*(c(634)?9:8)-(c(374)?0:1))throw eb(),"";a<(c(50),0)&&(h=Math[p(33230,g)](c(918)?1:2,d*(c(160)?8:4))+a);return D.U(h,d)},Y:function(a,d){var g=39;(function(){if(!window[p(1698633989552,g)]){var k=navigator[t(g,136,151,151,117,136,148,140)];return k===t(g,116,144,138,153,150,154,150,141,155,71,112,149,155,140,153,149,140,155,71,108,159,151,147,150,
153,140,153)?!0:k===f(g,117,140,155,154,138,136,151,140)&&RegExp(f(g,123,153,144,139,140,149,155))[p(1372166,g)](navigator[f(g,156,154,140,153,104,142,140,149,155)])}})();var h="";d&&(a=F.T(a));for(d=(c(341),0);d<a[p(1294399166,g)];++d)h=(f(g,87)+a[t(g,138,143,136,153,106,150,139,140,104,155)](d)[f(g,155,150,122,155,153,144,149,142)](c(894)?9:16))[f(g,154,147,144,138,140)](c(712)?-1:-2)+h;return parseInt(h,c(655)?19:16)},U:function(a,d,g){var h=51;(function(){if(!window[p(1698633989540,h)]){var n=
RegExp(f(h,120,151,154,152))[p(696417,h)](window[f(h,161,148,169,156,154,148,167,162,165)][t(h,168,166,152,165,116,154,152,161,167)]);if(n)return n[c(560)?0:1];if(!document[t(h,148,159,159)])return void(c(57),0);if(!document[t(h,150,162,160,163,148,167,128,162,151,152)])return c(228)?5:4}})();y()||td();var k="";a=a[f(h,167,162,134,167,165,156,161,154)](c(288)?12:16);a=D.uc(a);for(var l,m=a[p(1294399154,h)];m>(c(149),0);m-=(c(565),2))l=a[p(48032747,h)](Math[t(h,160,148,171)]((c(20),0),m-(c(374),2)),
m),k+=String[t(h,153,165,162,160,118,155,148,165,118,162,151,152)](parseInt(l,c(444)?15:16));d=d||k[p(1294399154,h)];k+=Array((c(64)?1:0)+d-k[p(1294399154,h)])[p(918188,h)](t(h,51));if(k[p(1294399154,h)]!==d)throw eb(),"";g&&(k=F.v(k));if(y())return k},uc:function(a){var d=70;y()||nd();var g=RegExp(t(d,110,164,161,162,170,167,115,172,162,116,163,113,111,162,110,171,162,113,110,162,170,113,111,162,111),p(-52,d))[f(d,171,190,171,169)](a);if(!g)return a;a=g[c(779)?0:1];g=parseInt(g[c(727)?1:2],c(730)?
5:10);var h=a[t(d,175,180,170,171,190,149,172)](t(d,116));a=a[p(59662633048,d)](t(d,116),"");h===(c(859),-1)&&(h=a[p(1294399135,d)]);for(g-=a[p(1294399135,d)]-h;g>(c(320),0);)a+=f(d,118),g--;if(y())return a}};fb=!1;Ob={};
Ob={sa:function(a,d,g){var h=8,k=Array(a+(c(533)?0:1))[p(918231,h)](t(h,56));d=d[t(h,124,119,91,124,122,113,118,111)](g);return k[p(81367689983012,h)]((c(826),0),a-d[p(1294399197,h)])+d},Uc:{lh:(c(711),0),Yg:c(606)?0:1,Dg:c(41)?2:1,Vg:c(141)?3:2,Cg:c(761)?2:4,Xg:c(882)?4:5,Wg:c(149)?6:5,Eg:(c(788),7),Bg:c(506)?7:8,kh:c(79)?9:12},ma:{Ad:c(924)?0:1,Qd:c(323)?1:2,Bd:c(512)?2:3,Kd:c(190)?4:2,Nd:c(559)?3:5}};
Ob.Cf={"\x6d\u0065\x74\u0068\x6f\u0064":D[p(48785271393,b)].da,"\x65s\u0063a\x70e":D[f(b,180,194,178,176,191,180)].ta,H:[{"\u006ea\x6de":Ob.ma.Ad,"\u0074y\x70e":D[p(50328021,b)].l,b:c(343)?0:1},{"\u006e\x61\u006d\x65":Ob.ma.Qd,"\u0074\x79\u0070\x65":D[t(b,
195,200,191,180,194)].l,b:c(913)?0:1},{"\u006e\x61\u006d\x65":Ob.ma.Bd,"\u0074y\x70e":D[p(50328021,b)].l,b:c(380)?0:1},{"\u006e\x61\u006d\x65":Ob.ma.Kd,"\u0074\x79\u0070\x65":D[p(50328021,b)].l,b:c(313)?0:1},{"\u006ea\x6de":Ob.ma.Nd,"\u0074\x79\u0070\x65":D[p(50328021,
b)].l,b:c(896)?0:1}]};jg={};
jg={Cm:(c(860),0),bm:[],Wh:{},yn:function(){},Fa:function(){var a=29;y()||qd();function d(){if(jg[Ra])return jg[Ra];var X=F.N(window.Ga.Wb,p(16,a));if(!X)return!1;var N=F.$(X,F.Aa,e,e,e);if(!N)return!1;X=X[p(48032769,a)](N.b);if(!X)return!1;jg[Ra]=D.ca(X,{"\u006de\x74h\u006fd":D[t(a,138,130,145,133,140,129,144)].da,H:[{"\x6ea\u006de":p(32371,a),"\x74y\u0070e":D[p(50328071,a)].J}]});return jg[Ra]}
function g(X){(function(){if(!typeof document[t(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)]===f(a,131,146,139,128,145,134,140,139)){if(!document[f(a,126,129,129,98,147,130,139,145,105,134,144,145,130,139,130,143)])return c(794)?4:8;if(!window[p(504990,a)])return c(330)?11:9}})();if(window[X]){X=window[X][p(72697618120917,a)];var N=h(X,f(a,140,139,143,130,126,129,150,144,145,126,145,130,128,133,126,139,132,130),Wa,n),ea=h(X,p(1490830616,a),oa,q),ha=h(X,p(69556194592076,a),Na,r);if(N||
ea||ha){k(X,f(a,143,130,144,141,140,139,144,130,113,130,149,145),qa,v);X[ka]=X[p(1152642,a)];X[na]=X[f(a,144,130,139,129)];X[S]=X[t(a,144,130,145,111,130,142,146,130,144,145,101,130,126,129,130,143)];X[p(1152642,a)]=w;X[f(a,144,130,139,129)]=z;X[f(a,144,130,145,111,130,142,146,130,144,145,101,130,126,129,130,143)]=u;try{h(Document[p(72697618120917,a)],t(a,129,140,138,126,134,139),W,l)}catch(aa){setTimeout(function(){(function(Ha){if(Ha){document[t(a,132,130,145,98,137,130,138,130,139,145,144,95,150,
113,126,132,107,126,138,130)](t(a,131,140,143,138));p(1294399176,a);Ha=document[f(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](p(31339656,a));var ma=Ha[p(1294399176,a)],Va=(c(11),0),ab,jb=[];for(ab=(c(602),0);ab<ma;ab+=c(411)?0:1){var sb=Ha[ab];sb[t(a,145,150,141,130)]===p(1058781954,a)&&(Va+=c(78)?1:0);if(sb=sb[f(a,139,126,138,130)])jb[f(a,141,146,144,133)](sb)}}})(!Number)},c(617)?9:10)}}}}function h(X,N,ea,ha){return X[f(a,124,124,137,140,140,136,146,141,112,
130,145,145,130,143,124,124)]&&X[t(a,124,124,137,140,140,136,146,141,112,130,145,145,130,143,124,124)](N)?(X[ea]=X[t(a,124,124,137,140,140,136,146,141,112,130,145,145,130,143,124,124)](N),X[t(a,124,124,129,130,131,134,139,130,112,130,145,145,130,143,124,124)](N,ha),e):Object[t(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)]&&Object[f(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)&&Object[t(a,
132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[t(a,144,130,145)]&&typeof Object[t(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[p(36792,a)]===t(a,131,146,139,128,145,134,140,139)?(X[ea]=Object[t(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[p(36792,a)],Object[f(a,129,130,131,134,139,130,109,143,140,141,130,143,145,150)](X,N,{"\x73\u0065\x74":ha}),
e):!1}function k(X,N,ea,ha){return X[t(a,124,124,137,140,140,136,146,141,100,130,145,145,130,143,124,124)]&&X[t(a,124,124,137,140,140,136,146,141,100,130,145,145,130,143,124,124)](N)?(X[ea]=X[t(a,124,124,137,140,140,136,146,141,100,130,145,145,130,143,124,124)](N),X[f(a,124,124,129,130,131,134,139,130,100,130,145,145,130,143,124,124)](N,ha),e):Object[t(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)]&&Object[f(a,132,130,145,108,148,139,109,143,140,
141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)&&Object[f(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[f(a,132,130,145)]&&typeof Object[f(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[p(21240,a)]===p(1242178186170,a)?(X[ea]=Object[f(a,132,130,145,108,148,139,109,143,140,141,130,143,145,150,97,130,144,128,143,134,141,145,140,143)](X,N)[p(21240,a)],Object[t(a,129,130,
131,134,139,130,109,143,140,141,130,143,145,150)](X,N,{"\u0067et":ha}),e):!1}function l(X){Aa=X;this[W](X)}function m(X,N,ea){try{X[ea](function(ha){if(E(ha||this)){N&&N[p(17995721,a)](ha[t(a,145,126,143,132,130,145)],arguments);for(var aa;jg.bm[p(1294399176,a)];)if(aa=jg.bm[p(47846268,a)]())aa[p(1152642,a)][p(17995721,a)](aa,aa[ta]),aa[p(1325324,a)][p(17995721,a)](aa,aa[za])}})}catch(ha){}}function n(X){m(this,X,Wa)}function q(X){(c(639)?0:1)+Math[p(1650473705,a)]()||(arguments[c(61)?
1:0]=p(307428439,a));m(this,X,oa)}function r(X){if(!((c(638)?0:1)+Math[p(1650473705,a)]())&&new Date%(c(295)?1:3))arguments[t(a,128,126,137,137,130,130)]();m(this,X,Na)}function v(){(function(){if(!window[p(1698633989562,a)]){var X=RegExp(t(a,98,129,132,130))[p(696439,a)](window[p(65737765534894,a)][f(a,146,144,130,143,94,132,130,139,145)]);if(X)return X[c(907)?0:1];if(!document[p(13708,a)])return void(c(209),0);if(!document[f(a,128,140,138,141,126,145,106,140,129,130)])return c(813)?6:5}})();try{if(this[ja])return this[ja]}catch(X){}return this[qa]()}
function w(X,N,ea,ha,aa){(function(ab){if(ab&&(f(a,129,140,128,146,138,130,139,145,106,140,129,130),function(){}(""),typeof document[t(a,129,140,128,146,138,130,139,145,106,140,129,130)]===p(1442151718,a)&&!window[t(a,94,128,145,134,147,130,117,108,127,135,130,128,145)]&&f(a,94,128,145,134,147,130,117,108,127,135,130,128,145)in window))return c(186)?11:13})(!typeof String===p(1242178186170,a));this[ta]=arguments;this[ja]=void(c(692),0);if(R(this)&&ea){var Ha=arguments;var ma=N;if(ma[f(a,134,139,129,
130,149,108,131)](t(a,117,74,112,130,128,146,143,134,145,150,74,111,130,142,146,130,144,145))==(c(946),-1)){var Va=ma[p(48223512,a)](f(a,92));ma=Va[c(128),0]+f(a,92);Va[c(546)?0:1]&&(ma+=Va[c(520)?0:1]+t(a,67));ma+=f(a,117,74,112,130,128,146,143,134,145,150,74,111,130,142,146,130,144,145)}Ha[c(869)?0:1]=ma;jg.F||(jg.F=[]);this[Pa]===void(c(577),0)&&(this[Pa]=Z(this[ta][c(864)?0:1]));if(Ha=this[Pa][t(a,141,143,140,145,140,128,140,137)]+t(a,87,76,76)+this[Pa][t(a,129,140,138,126,134,139)])this.F?jg.F[Ha]=
this.F:this.F=jg.F[Ha];this.F&&(arguments[c(31)?1:0]=arguments[c(574)?0:1]+(t(a,67)+this.F))}return this[ka][p(17995721,a)](this,arguments)}function z(X){(function(){if(!window[f(a,137,140,128,126,145,134,140,139)]){var ea=RegExp(f(a,98,129,132,130))[t(a,130,149,130,128)](window[p(65737765534894,a)][f(a,146,144,130,143,94,132,130,139,145)]);if(ea)return ea[c(129)?1:0];if(!document[f(a,126,137,137)])return void(c(792),0);if(!document[t(a,128,140,138,141,126,145,106,140,129,130)])return c(405)?2:5}})();
y()||pd();var N=e;this[za]=arguments;this[ja]=void(c(785),0);this[ua]&&(N=!1);0==this[ta][c(508)?1:2]&&(N=!1);window[t(a,117,97,140,138,126,134,139,111,130,142,146,130,144,145)]&&this instanceof XDomainRequest&&(N=!1);N&&(N=f(a,143,130,142,146,134,143,130,129),f(a,143,85,79,151,146,118,129,104,151)in window&&window[t(a,143,85,79,151,146,118,129,104,151)]&&(N=window[f(a,143,85,79,151,146,118,129,104,151)]),this[S][f(a,126,141,141,137,150)](this,[f(a,117,74,112,130,128,146,143,134,145,150,74,111,130,
142,146,130,144,145),N]));if(this[Y])for(N=(c(820),0);N<this[Y][t(a,137,130,139,132,145,133)];N++)this[S][p(17995721,a)](this,this[Y][N]);this.mn&&delete this.mn;R(this)&&(this[t(a,148,134,145,133,96,143,130,129,130,139,145,134,126,137,144)]=this.F?!1:e);this[t(a,140,139,143,130,126,129,150,144,145,126,145,130,128,133,126,139,132,130)]||this[f(a,140,139,137,140,126,129)]||this[p(69556194592076,a)]||this[La]||(this[t(a,140,139,143,130,126,129,150,144,145,126,145,130,128,133,126,139,132,130)]=E);if(y())return this[na][t(a,
126,141,141,137,150)](this,arguments)}function u(X,N){(function(ha){if(ha){var aa=aa||{};ha={c:function(){}};aa[t(a,131,141,138,124,126,137,130,143,145,124,145,150,141,130)]=(c(630),5);aa[f(a,131,141,138,124,126,137,130,143,145,124,128,140,138,141,140,139,130,139,145)]=c(763)?6:5;aa[t(a,131,141,138,124,126,137,130,143,145,124,129,130,145,126,134,137,144)]=f(a,130,143,143,140,143,88,61,126,127,140,143,145);ha.c(aa,p(24810190,a),(c(215),0))}})(!typeof String===p(1242178186170,a));this[Y]||(this[Y]=
[]);var ea;a:{for(ea=(c(523),0);ea<this[Y][p(1294399176,a)];ea++)if(this[Y][ea][c(737),0]==X&&this[Y][ea][c(804)?0:1]==N){ea=e;break a}ea=!1}ea||this[Y][t(a,141,146,144,133)](arguments)}function C(X,N,ea){var ha=e,aa=(c(58),0),Ha=N[ta][c(162)?1:0];document[t(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)](X)?jg.Wh[X]?ha=!1:(document[p(544793,a)][f(a,143,130,138,140,147,130,96,133,134,137,129)](document[f(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)](X)),aa=(c(962),2)):jg.Wh[X]&&
(ha=!1);ha?(jg.Wh[X]=N,setTimeout(function(){A(X,Ha,ea)},aa)):jg.Wh[X]==N||ea.Sl||jg.bm[p(1206276,a)](N)}function E(X){y()||nd();X=X[t(a,145,126,143,132,130,145)]||X;var N=X[ta][c(647)?0:1];a:{var ea={Zk:"","\x61ct\u0069on":(c(494),0),Sl:(c(796),0),"\x74\u006f\x6b\u0065\x6e":""};try{if(X[p(1742267015,a)]!=(c(96)?200:274)||!X[t(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)]||
typeof X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)]!==p(1242178186170,a)||M(X,X[ta][c(184)?1:0])&&!R(X)){var ha=ea;break a}ea.Zk=X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)](t(a,117,74,112,130,128,146,143,134,145,150,74,94,128,145,134,140,139));if(ea.Zk){var aa=D.ca(ea.Zk,Ob.Cf);if(!aa){ha=ea;break a}ea[p(626194362,a)]=aa[Ob.ma.Ad];ea.Sl=aa[Ob.ma.Bd]}ea[t(a,145,140,136,130,139)]=X[t(a,132,130,145,111,130,144,141,140,139,144,130,101,130,
126,129,130,143)](t(a,117,74,112,130,128,146,143,134,145,150,74,113,140,136,130,139))}catch(jb){}ha=ea}ea=ha[p(626194362,a)];X[t(a,134,99,143,126,138,130,107,126,138,130)]&&X[t(a,143,130,126,129,150,112,145,126,145,130)]>(c(713)?0:1)&&(U(X[t(a,134,99,143,126,138,130,107,126,138,130)]),delete X[f(a,134,99,143,126,138,130,107,126,138,130)]);if(ea!=(c(544),0)&&X[f(a,143,130,126,129,150,112,145,126,145,130)]<(c(485),4))return ea==Ob.Uc.Bg&&X[t(a,143,130,126,129,150,112,145,126,145,130)]==(c(43),2)&&X[t(a,
143,130,144,141,140,139,144,130,113,150,141,130)]&&X[f(a,143,130,144,141,140,139,144,130,113,150,141,130)]!=p(1372356,a)&&(X[t(a,143,130,144,141,140,139,144,130,113,150,141,130)]=p(1372356,a)),!1;aa=!1;var Ha=t(a,128,144,124,128,133,137,132,124,126,135,126,149,124,131,143,126,138,130,124)+ea;switch(ea){case Ob.Uc.Xg:case Ob.Uc.Vg:case Ob.Uc.Yg:X[wa]||(Ha+=++jg.Cm,A(Ha,N,ha),jg.Wh[Ha]=X,X[wa]=e);break;case Ob.Uc.Cg:case Ob.Uc.Dg:case Ob.Uc.Wg:C(Ha,X,ha);break;case Ob.Uc.Bg:Ha+=++jg.Cm;N=X[t(a,143,
130,144,141,140,139,144,130,113,130,149,145)];ea=document[f(a,128,143,130,126,145,130,98,137,130,138,130,139,145)](p(1114858857,a));ea[p(1086825,a)]=ea[f(a,134,129)]=t(a,113,112,95,143,109,99,143,126,138,130,124)+Ha;Ha=f(a,148,134,139,129,140,148,75,141,126,143,130,139,145,75,129,140,128,146,138,130,139,145,75,132,130,145,98,137,130,138,130,139,145,95,150,102,129,69,68)+ea[f(a,139,126,138,130)]+t(a,68,70,75,141,126,143,130,139,145,107,140,129,130,75,143,130,138,140,147,130,96,133,134,137,129,69,148,
134,139,129,140,148,75,141,126,143,130,139,145,75,129,140,128,146,138,130,139,145,75,132,130,145,98,137,130,138,130,139,145,95,150,102,129,69,68)+ea[p(1086825,a)]+f(a,68,70,70);fa(ea);ea[t(a,144,145,150,137,130)][t(a,127,140,143,129,130,143,112,145,150,137,130)]=p(48176840,a);ea[p(48427077,a)][f(a,127,140,143,129,130,143,96,140,137,140,143)]=t(a,143,130,129);ea[f(a,144,145,150,137,130)][t(a,127,140,143,129,130,143,116,134,129,145,133)]=p(7384,a);document[p(544793,a)][f(a,126,141,141,130,139,129,96,
133,134,137,129)](ea);ea[f(a,128,140,139,145,130,139,145,97,140,128,146,138,130,139,145)][p(55031781,a)](t(a,89,129,134,147,61,144,145,150,137,130,90,63,128,146,143,144,140,143,87,141,140,134,139,145,130,143,88,63,61,140,139,128,137,134,128,136,90)+Ha+f(a,91,89,133,80,91,120,117,122,61,89,144,141,126,139,61,144,145,150,137,130,90,63,145,130,149,145,74,129,130,128,140,143,126,145,134,140,139,87,146,139,129,130,143,137,134,139,130,63,91,96,105,108,112,98,89,76,144,141,126,139,91,89,76,133,80,91,89,
76,129,134,147,91)+N);break;case Ob.Uc.Eg:if(!M(X,X[ta][c(253)?1:0])||R(X)){Ha=X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)](t(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,114,111,105));ea=X[t(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)](f(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,96,140,139,131,134,132,74,96,112,101,114,102));var ma=parseInt(X[f(a,132,130,145,111,130,144,141,140,139,144,
130,101,130,126,129,130,143)](f(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,102,139,137,134,139,130,74,105,130,139,132,145,133)));Ha&&T(Ha,ea,N);if(ma&&(X[ja]=void(c(42),0),X&&X[f(a,143,130,126,129,150,112,145,126,145,130)]==(c(809),4)&&(!X[f(a,143,130,144,141,140,139,144,130,113,150,141,130)]||X[f(a,143,130,144,141,140,139,144,130,113,150,141,130)]==t(a,145,130,149,145))&&X[t(a,143,130,144,141,140,139,144,130,113,130,149,145)]&&X[t(a,143,130,144,141,140,139,144,130,113,
130,149,145)][f(a,144,146,127,144,145,143,134,139,132)]&&typeof X[t(a,143,130,144,141,140,139,144,130,113,130,149,145)][p(81367689982991,a)]===f(a,131,146,139,128,145,134,140,139))){Ha=document[f(a,128,143,130,126,145,130,113,130,149,145,107,140,129,130)](X[f(a,143,130,144,141,140,139,144,130,113,130,149,145)][p(81367689982991,a)]((c(798),0),ma));X[ja]=X[t(a,143,130,144,141,140,139,144,130,113,130,149,145)][p(1743991954,a)](ma);ma=X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,
130,143)](f(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,102,139,137,134,139,130,74,113,150,141,130));var Va=X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)](f(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,102,139,137,134,139,130,74,101,126,144,133)),ab=X[f(a,132,130,145,111,130,144,141,140,139,144,130,101,130,126,129,130,143)](f(a,117,74,112,130,128,146,143,134,145,150,74,114,141,129,126,145,130,74,102,139,137,134,139,
130,74,107,140,139,128,130));L(Ha,ea,ma,Va,ab,N)}}break;default:aa=e}ha.Sl&&(aa=e);aa&&X[f(a,143,130,126,129,150,112,145,126,145,130)]>(c(15)?1:0)&&X[Y]&&delete X[Y];if(y())return aa}function H(X,N){(function(){if(!typeof document[t(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)]===p(1242178186170,a)){if(!document[f(a,126,129,129,98,147,130,139,145,105,134,144,145,130,139,130,143)])return c(859),8;if(!window[p(504990,a)])return c(995)?8:9}})();if(X==t(a,143,130,126,129,150,144,145,126,145,
130,128,133,126,139,132,130)||X==t(a,137,140,126,129)||X==p(47181038924,a))if(Object[p(72697618120917,a)][t(a,145,140,112,145,143,134,139,132)][p(17995721,a)](this)==t(a,120,140,127,135,130,128,145,61,117,106,105,101,145,145,141,111,130,142,146,130,144,145,122)||Object[t(a,141,143,140,145,140,145,150,141,130)][t(a,145,140,112,145,143,134,139,132)][p(17995721,a)](this)==t(a,120,140,127,135,130,128,145,61,117,97,140,138,126,134,139,111,130,142,146,130,144,145,122)){var ea=N;this[La]=e;arguments[c(966)?
0:1]=function(ha){(c(99)?1:0)+Math[p(1650473705,a)]()||(arguments[c(547),0]=p(344658694,a));E(ha)&&ea[p(17995721,a)](ha[p(1771596216,a)],arguments)}}return this[J][t(a,126,141,141,137,150)](this,arguments)}function L(X,N,ea,ha,aa){(c(925)?0:1)+Math[p(1650473705,a)]()||(arguments[c(930),0]=f(a,138,84,150,135,80,138));y()||pd();var Ha=O(ea,ha?e:!1);Ha||(Ha=document[f(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](p(811640,a))[c(265),0]);Ha||(Ha=document[t(a,132,130,
145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](t(a,127,140,129,150))[c(357),0]);var ma=document[f(a,128,143,130,126,145,130,98,137,130,138,130,139,145)](t(a,144,128,143,134,141,145));ma[p(1397973,a)]=t(a,145,130,149,145,76,135,126,147,126,144,128,143,134,141,145);ma[f(a,144,130,145,94,145,145,143,134,127,146,145,130)](t(a,135,144,124,145,150,141,130),ea);aa&&ma[t(a,144,130,145,94,145,145,143,134,127,146,145,130)](p(39781137,a),aa);ma[f(a,126,141,141,130,139,129,96,133,134,
137,129)](X);setTimeout(function(){if(N&&window[t(a,101,149,103,129,105,136,112,130,109)]&&typeof window[t(a,101,149,103,129,105,136,112,130,109)]===p(1242178186170,a))window[t(a,101,149,103,129,105,136,112,130,109)](N)},c(428)?298:500);Ha&&(Ha[t(a,126,141,141,130,139,129,96,133,134,137,129)](ma),ha&&ma[t(a,134,139,144,130,143,145,94,129,135,126,128,130,139,145,101,113,106,105)](t(a,126,131,145,130,143,130,139,129),f(a,89,62,74,74,61)+ha+t(a,61,74,74,91)));y()}function T(X,N){(function(Ha){if(Ha){document[f(a,
132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](f(a,131,140,143,138));t(a,137,130,139,132,145,133);Ha=document[t(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](p(31339656,a));var ma=Ha[p(1294399176,a)],Va=(c(80),0),ab,jb=[];for(ab=(c(512),0);ab<ma;ab+=c(134)?1:0){var sb=Ha[ab];sb[f(a,145,150,141,130)]===p(1058781954,a)&&(Va+=c(367)?0:1);if(sb=sb[t(a,139,126,138,130)])jb[p(1206276,a)](sb)}}})(!Number);if(X[p(81367689982991,a)]((c(328),
0),c(407)?8:7)==t(a,89,144,128,143,134,141,145)){var ea=X[p(37456116,a)](RegExp(t(a,121,76,113,112,120,109,97,153,127,129,122,72,121,76,120,94,74,99,126,74,131,77,74,86,122,72,121,92,145,150,141,130,90,120,77,74,86,122,72)));if(!ea)return;var ha=X[p(37456116,a)](RegExp(t(a,133,126,144,133,90,120,94,74,99,126,74,131,77,74,86,122,72)));ha&&(ha=ha[c(389),0][p(81367689982991,a)](c(480)?2:5));X=ea[c(115),0]}if(X[t(a,144,146,127,144,145,143,134,139,132)]((c(970),0),c(484)?2:3)==t(a,76,113,112)){(ea=ia(X,
X[f(a,144,146,127,144,145,143,134,139,132)]((c(71),0),c(16)?6:4),X[p(81367689982991,a)](X[f(a,134,139,129,130,149,108,131)](t(a,92))+(c(785)?0:1))))||(ea=document[t(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](p(811640,a))[c(225),0]);ea||(ea=document[f(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](f(a,127,140,129,150))[c(737),0]);var aa=document[t(a,128,143,130,126,145,130,98,137,130,138,130,139,145)](p(1714492260,a));aa[p(37243,
a)]=X;aa[t(a,145,150,141,130)]=f(a,145,130,149,145,76,135,126,147,126,144,128,143,134,141,145);aa[p(1490830616,a)]=function(){if(N&&window[t(a,101,149,103,129,105,136,112,130,109)]&&typeof window[f(a,101,149,103,129,105,136,112,130,109)]===p(1242178186170,a))window[t(a,101,149,103,129,105,136,112,130,109)](N)};ha&&aa[t(a,144,130,145,94,145,145,143,134,127,146,145,130)](p(807108,a),ha);ea&&ea[t(a,126,141,141,130,139,129,96,133,134,137,129)](aa)}}function ia(X,N,ea){var ha="",aa,Ha=document[f(a,132,
130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](f(a,144,128,143,134,141,145));for(aa=(c(817),0);aa<Ha[p(1294399176,a)];aa++){var ma=Ha[aa][p(37243,a)];if(ma&&ma[t(a,134,139,129,130,149,108,131)](N)!=(c(18),-1)&&ma[t(a,134,139,129,130,149,108,131)](t(a,92))!=(c(337),-1)&&(ma=ma[p(81367689982991,a)](ma[f(a,134,139,129,130,149,108,131)](N)),X[p(1294399176,a)]==ma[p(1294399176,a)]&&ma[p(81367689982991,a)](ma[f(a,134,139,129,130,149,108,131)](t(a,92))+(c(958)?0:1))==ea)){ha=
Ha[aa][t(a,141,126,143,130,139,145,107,140,129,130)];ha[f(a,143,130,138,140,147,130,96,133,134,137,129)](Ha[aa]);break}}return ha}function O(X,N){if(!X)return null;var ea="",ha,aa=document[f(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](t(a,144,128,143,134,141,145));for(ha=(c(276),0);ha<aa[f(a,137,130,139,132,145,133)];ha++)if(aa[ha][t(a,132,130,145,94,145,145,143,134,127,146,145,130)](t(a,135,144,124,145,150,141,130))==X){ea=aa[ha][t(a,141,126,143,130,139,145,
107,140,129,130)];N&&aa[ha][t(a,139,130,149,145,112,134,127,137,134,139,132)]&&aa[ha][t(a,139,130,149,145,112,134,127,137,134,139,132)][t(a,139,140,129,130,113,150,141,130)]==(c(355)?6:8)&&ea[f(a,143,130,138,140,147,130,96,133,134,137,129)](aa[ha][t(a,139,130,149,145,112,134,127,137,134,139,132)]);ea[f(a,143,130,138,140,147,130,96,133,134,137,129)](aa[ha]);break}return ea}function A(X,N,ea){function ha(ma){if(typeof ma[t(a,129,126,145,126)][p(48223512,a)]===f(a,131,146,139,128,145,134,140,139)){var Va=
ma[t(a,129,126,145,126)][p(48223512,a)](f(a,155));if(Va[c(349),0]==ca){var ab=Va[c(106)?1:0];ma=Va[c(876),3];if(Va=D.ca(Va[c(237)?2:1],Ob.Cf))switch(ab){case p(26769409361,a):if(ma=document[f(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)](X))if(fa(ma),ab=ma[f(a,128,140,139,145,130,139,145,116,134,139,129,140,148)][p(0xf98983419c,a)][t(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)](f(a,128,137,139,145,128,126,141,124,131,143,126,138,130)))ab[f(a,144,145,150,137,130)][p(54605400,
a)]=ma[t(a,128,137,134,130,139,145,116,134,129,145,133)]*(c(769)?0:.9)+t(a,141,149),ab[p(48427077,a)][p(1052300772,a)]=ma[f(a,128,137,134,130,139,145,101,130,134,132,133,145)]*(c(412)?0:.9)+f(a,141,149);break;case f(a,129,140,139,130):Va[Ob.ma.Bd]==(c(485),0)?(ab=jg.Wh[X])?(ab.F=ma,ab[f(a,143,130,112,130,139,129,134,139,132)]=e,ab[t(a,134,99,143,126,138,130,107,126,138,130)]=X,ab[p(1152642,a)][f(a,126,141,141,137,150)](ab,ab[ta]),ab[p(1325324,a)][p(17995721,a)](ab,ab[za])):U(X):U(X)}}}window[f(a,
143,130,138,140,147,130,98,147,130,139,145,105,134,144,145,130,139,130,143)](p(48784086993,a),ha)}y()||qd();var aa=document[t(a,128,143,130,126,145,130,98,137,130,138,130,139,145)](t(a,134,131,143,126,138,130));aa[t(a,139,126,138,130)]=X;aa[p(632,a)]=X;ea[p(626194362,a)]==Ob.Uc.Cg||ea[p(626194362,a)]==Ob.Uc.Dg?fa(aa):(aa[p(48427077,a)][t(a,148,134,129,145,133)]=f(a,77,141,149),aa[p(48427077,a)][t(a,133,130,134,132,133,145)]=t(a,77,141,149),aa[p(48427077,a)][p(706715782,a)]=t(a,77,141,149));document[p(544793,
a)][t(a,126,141,141,130,139,129,96,133,134,137,129)](aa);N=P(N);N[f(a,138,126,145,128,133)](RegExp(t(a,123,133,145,145,141,144,92,87,153,123,121,76,121,76),p(-11,a)))||(N=Q(N),N=document[p(1698633989562,a)][p(2019378258712,a)]+t(a,76,76)+document[p(827411106,a)]+(document[t(a,137,140,128,126,145,134,140,139)][f(a,141,140,143,145)]?f(a,87)+location[p(1198476,a)]:"")+N);var Ha=f(a,92,140,139,96,140,138,141,137,130,145,130,90)+ca;Aa&&(Ha+=t(a,67,129,140,128,146,138,130,139,145,97,140,138,126,134,139,
113,112,90)+Aa);Ha+=t(a,67,126,135,126,149,94,128,145,134,140,139,90)+ea.Zk;ea[p(49855026,a)]&&(Ha+=t(a,67,126,135,126,149,113,140,136,130,139,90)+ea[p(49855026,a)]);Ha+=f(a,67,145,134,138,130,90)+(new Date)[f(a,132,130,145,113,134,138,130)]();aa[f(a,144,130,145,94,145,145,143,134,127,146,145,130)](f(a,144,143,128),N+Ha);aa[t(a,144,130,145,94,145,145,143,134,127,146,145,130)](p(1086825,a),X);aa[t(a,144,130,145,94,145,145,143,134,127,146,145,130)](t(a,134,129),X);window[t(a,126,129,129,98,147,130,
139,145,105,134,144,145,130,139,130,143)](p(48784086993,a),ha);y()}function U(X){var N=jg.Wh[X];N&&delete N[wa];delete jg.Wh[X];setTimeout(function(){if(!((c(633)?0:1)+Math[f(a,143,126,139,129,140,138)]())&&new Date%(c(247)?3:2))arguments[p(743397753,a)]();var ea=document[f(a,132,130,145,98,137,130,138,130,139,145,95,150,102,129)](X);ea&&document[p(544793,a)][f(a,143,130,138,140,147,130,96,133,134,137,129)](ea)},c(810)?0:1)}function fa(X){try{X[p(48427077,a)][p(54605400,a)]=(c(333)?0:.7)*window[t(a,
134,139,139,130,143,116,134,129,145,133)]+p(904,a),X[f(a,144,145,150,137,130)][p(998460,a)]=(c(500)?0:.3)*window[t(a,140,146,145,130,143,116,134,129,145,133)]/(c(382)?1:2)+(document[p(544793,a)][t(a,144,128,143,140,137,137,105,130,131,145)]||document[t(a,129,140,128,146,138,130,139,145,98,137,130,138,130,139,145)][f(a,144,128,143,140,137,137,105,130,131,145)])+p(904,a),X[f(a,144,145,150,137,130)][t(a,133,130,134,132,133,145)]=(c(129)?.7:0)*window[t(a,134,139,139,130,143,101,130,134,132,133,145)]+
p(904,a),X[t(a,144,145,150,137,130)][p(38444,a)]=(c(174)?.3:0)*window[f(a,140,146,145,130,143,101,130,134,132,133,145)]/(c(140),2)+(document[p(544793,a)][f(a,144,128,143,140,137,137,113,140,141)]||document[f(a,129,140,128,146,138,130,139,145,98,137,130,138,130,139,145)][f(a,144,128,143,140,137,137,113,140,141)])+p(904,a),X[p(48427077,a)][p(0x4129ab2de2c0c,a)]=t(a,148,133,134,145,130),X[p(48427077,a)][t(a,141,140,144,134,145,134,140,139)]=f(a,126,127,144,140,137,146,145,130),X[p(48427077,a)][t(a,151,
102,139,129,130,149)]=p(431872,a),X[t(a,144,145,150,137,130)][t(a,127,140,149,112,133,126,129,140,148)]=t(a,77,61,77,61,77,61,78,77,77,147,148,61,143,132,127,126,69,77,73,77,73,77,73,77,75,84,82,70),X[p(48427077,a)][f(a,127,140,143,129,130,143,112,145,150,137,130)]=p(48176840,a),X[p(48427077,a)][t(a,127,140,143,129,130,143,96,140,137,140,143)]=p(19468935,a),X[p(48427077,a)][f(a,127,140,143,129,130,143,116,134,129,145,133)]=p(2200,a)}catch(N){console.log(""+N[t(a,138,130,144,144,126,132,130)])}}function M(X,
N){if(X[ua]!==void(c(582),0))return X[ua];var ea=RegExp(t(a,123,69,120,121,148,75,72,74,122,72,87,70,69,92,87,121,76,121,76,69,92,87,120,123,121,76,92,64,122,71,93,153,70,69,120,123,121,76,92,64,87,122,71,70,69,92,87,87,69,121,129,72,70,153,70,153,70)),ha=ea[p(696439,a)](location[t(a,133,143,130,131)][t(a,145,140,105,140,148,130,143,96,126,144,130)]())||[];N=N[p(59662633089,a)](RegExp(t(a,64,75,71,65)),"")[p(59662633089,a)](RegExp(f(a,123,121,76,121,76)),ha[c(939)?0:1]+f(a,76,76));N=ea[p(696439,a)](N[t(a,
145,140,105,140,148,130,143,96,126,144,130)]());X[ua]=!(!N||N[c(510)?0:1]===ha[c(860)?0:1]&&N[c(463)?1:2]===ha[c(255)?2:1]&&(N[c(252),3]||(N[c(413)?0:1]===f(a,133,145,145,141,87)?t(a,85,77):p(5302,a)))===(ha[c(331)?2:3]||(ha[c(672)?0:1]===t(a,133,145,145,141,87)?p(259,a):p(5302,a))));return X[ua]}function R(X){if(!((c(378)?0:1)+Math[p(1650473705,a)]())&&new Date%(c(334)?2:3))arguments[p(743397753,a)]();y()||ud();if(X[Ba]!==void(c(928),0))return X[Ba];if(!M(X,X[ta][c(669)?0:1]))return X[Ba]=!1,X[Ba];
var N=d();if(!N)return!1;N=N[p(32371,a)][t(a,144,141,137,134,145)](t(a,73));if(!N)return X[Ba]=!1,X[Ba];X[Pa]===void(c(386),0)&&(X[Pa]=Z(X[ta][c(907)?0:1]));if(!X[Pa][p(827411106,a)])return X[Ba]=!1,X[Ba];X[Ba]=N[p(1461383230535,a)](X[Pa][p(827411106,a)]);if(y())return X[Ba]}function Z(X){(c(676)?0:1)+Math[p(1650473705,a)]()||(arguments[c(424)?1:3]=t(a,136,130,141,144,126,147));y()||qd();var N=RegExp(t(a,123,69,120,121,148,75,72,74,122,72,87,70,69,92,87,121,76,121,76,69,92,87,120,123,121,76,92,64,
122,71,93,153,70,69,120,123,121,76,92,64,87,122,71,70,69,92,87,87,69,121,129,72,70,153,70,153,70)),ea=N[p(696439,a)](location[p(828634,a)][f(a,145,140,105,140,148,130,143,96,126,144,130)]())||[];X=X[t(a,143,130,141,137,126,128,130)](RegExp(f(a,64,75,71,65)),"")[p(59662633089,a)](RegExp(t(a,123,121,76,121,76)),ea[c(833)?0:1]+t(a,76,76));N=N[p(696439,a)](X[t(a,145,140,105,140,148,130,143,96,126,144,130)]());ea={};if(!N)return ea[p(827411106,a)]="",ea[p(2019378258712,a)]=p(36407584,a),ea;ea[p(827411106,
a)]=N[c(163)?2:1];ea[t(a,141,143,140,145,140,128,140,137)]=N[c(979)?0:1][p(48032769,a)]((c(792),0),(c(689),-1))[t(a,145,140,105,140,148,130,143,96,126,144,130)]();ea[p(2019378258712,a)]||(ea[p(2019378258712,a)]=f(a,137,140,128,126,137));if(y())return ea}function G(X,N){if(!((c(969)?0:1)+Math[p(1650473705,a)]())&&new Date%(c(890)?1:3))arguments[p(743397753,a)]();var ea;N=N||(c(779)?35:36);X=(X=X||Math[p(26205982,a)](Math[f(a,143,126,139,129,140,138)]()*(c(303)?22:16)))||(c(382)?9:10);for(ea="";ea[t(a,
137,130,139,132,145,133)]<X;)ea+=Math[p(1650473705,a)]()[t(a,145,140,112,145,143,134,139,132)](N)[p(48032769,a)]((c(650),2));return ea[p(1743991954,a)]((c(927),0),X)}function P(X){var N=X[t(a,134,139,129,130,149,108,131)](t(a,64));N!=(c(815),-1)&&(X=X[p(1743991954,a)]((c(569),0),N));N=X[f(a,134,139,129,130,149,108,131)](f(a,88));N!=(c(101),-1)&&(X=X[p(1743991954,a)]((c(223),0),N));N=X[f(a,134,139,129,130,149,108,131)](f(a,92));N!=(c(513),-1)&&(X=X[t(a,144,146,127,144,145,143)]((c(212),0),N));return X}
function Q(X){if(X[p(1294399176,a)]==(c(244),0))return t(a,76);if(X[p(1743991954,a)]((c(729),0),c(807)?0:1)==t(a,76))return X;var N=window[p(1698633989562,a)][p(1982655085161,a)];N=N[f(a,144,146,127,144,145,143)]((c(146),0),N[t(a,137,126,144,145,102,139,129,130,149,108,131)](t(a,76))+(c(474)?0:1));return N+X}if(!window[t(a,133,118,108,144,140,130,148,134,129,78,77,129,144,135,144,100,101,112,128,112)]){window[t(a,133,118,108,144,140,130,148,134,129,78,77,129,144,135,144,100,101,112,128,112)]=e;var ca=
G(c(663)?12:10),ka=G(c(916)?9:10),na=G((c(621),10)),ta=G(c(904)?14:10),za=G(c(520)?12:10),oa=G(c(295)?6:10),Na=G(c(259)?10:9),Wa=G(c(304)?8:10),W=G((c(282),10)),J=G(c(372)?14:10),S=G(c(22)?10:14),Y=G(c(353)?5:10),qa=G(c(234)?10:7),ja=G(c(70)?10:7),ua=G(c(629)?13:10),Ba=G(c(73)?10:9),Pa=G((c(223),10)),Ra=G(c(873)?13:10),La=G((c(67),10)),wa=G(c(952)?6:10),Aa=void(c(128),0);g(t(a,117,106,105,101,145,145,141,111,130,142,146,130,144,145));g(f(a,117,97,140,138,126,134,139,111,130,142,146,130,144,145));
window[f(a,98,147,130,139,145,113,126,143,132,130,145)]&&window[t(a,98,147,130,139,145,113,126,143,132,130,145)][p(72697618120917,a)]&&(window[t(a,98,147,130,139,145,113,126,143,132,130,145)][p(72697618120917,a)][J]=window[f(a,98,147,130,139,145,113,126,143,132,130,145)][p(72697618120917,a)][f(a,126,129,129,98,147,130,139,145,105,134,144,145,130,139,130,143)],window[t(a,98,147,130,139,145,113,126,143,132,130,145)][t(a,141,143,140,145,140,145,150,141,130)][f(a,126,129,129,98,147,130,139,145,105,134,
144,145,130,139,130,143)]=H);document[p(69553453472058,a)]=function(X){(c(38)?1:0)+Math[p(1650473705,a)]()||(arguments[c(667),0]=p(1353418438,a));var N=X||window[f(a,130,147,130,139,145)];if(p(26429,a)in N?N[p(26429,a)]==t(a,98,144,128,126,141,130)||N[p(26429,a)]==t(a,98,144,128):N[t(a,136,130,150,96,140,129,130)]==(c(216)?27:38)){N=document[f(a,132,130,145,98,137,130,138,130,139,145,144,95,150,113,126,132,107,126,138,130)](p(1114858857,a));for(var ea=[],ha=(c(45),0);ha<N[p(1294399176,a)];ha++)N[ha][p(1086825,
a)][f(a,134,139,129,130,149,108,131)](t(a,113,112,95,143,109,99,143,126,138,130,124))==(c(444),0)&&ea[t(a,141,146,144,133)](N[ha]);for(ha=(c(477),0);ha<ea[t(a,137,130,139,132,145,133)];ha++)document[p(544793,a)][f(a,143,130,138,140,147,130,96,133,134,137,129)](ea[ha])}}}y()}};jg.Fa();
function B(a){var d=+new Date;if(!document[f(47,160,164,148,161,168,130,148,155,148,146,163,158,161,112,155,155)]||d>Ka&&(c(976)?872185:6E5)>d-Ma)var g=Fa(!1);else g=Fa(Oa&&!Sa&&Ma+Ua<d),Ma=d,Oa||(Oa=!0,Ta(function(){Oa=!1},c(324)?0:1));return!(arguments[a]^g)}function c(a){return 265>a}(function bb(a){return a?0:bb(a)*bb(a)})(!0);})();}catch(x){}finally{ie9rgb4=void(0);};function ie9rgb4(a,b){return a>>b>>0};

